Complexity of Membership and Non-Emptiness Problems in Unbounded Memory Automata

We study the complexity relationship between three models of unbounded memory automata: nu-automata ($\nu$-A), Layered Memory Automata (LaMA)and History-Register Automata (HRA). These are all extensions of finite state automata with unbounded memory over infinite alphabets. We prove that the membership problem is NP-complete for all of them, while they fall into different classes for what concerns non-emptiness. The problem of non-emptiness is known to be Ackermann-complete for HRA, we prove that it is PSPACE-complete for $\nu$-A.

==> Damien_preuves_pspace.tex <==
\begin{lemma}\label{lem:accepted-pumpable}
Let $\simpli(A)$ be simplified $\nu$-automaton and $w$ a simplified input word recognized by this automaton. If the length of $w$ is greater than $|Q|2^{|K|}+1$, then $w$ is pumpable. If $w$ is accepted by a sequence of transitions of length greater than $|Q|2^{|K|}+1$, then the sequence is pumpable.
\end{lemma}
%\begin{lemma}\label{lem:accepted-pumpable}
%Considérons un $\nu$-automate simplifié et un mot simplifié $w$ reconnu par cet automate. Si ce mot est plus long que $|Q|2^{|K|}+1$ dans ce cas il est pompable. Si ce mot est accepté par une séquence de transition de taille plus de $|Q|2^{|K|}+1$ alors la séquence est pompable. 

%NOTE: En fait, j'ai besoin par la suite que la séquence de transition soit bornée, si on croise une boucle avec que des resets, il faut aussi montrer que ceux-ci sont inutiles.
%\end{lemma}


\begin{proof}
Let $w$ be a simplified word accepted by a simplified $\nu$-automaton $A$.
Let $\sigma$ be a sequence of transitions accepting $w$ of length at least $|Q|2^{|M|+|K|}+1$.
In this case the sequence of  configurations encountered during the reading of $w$ contains contains two identical ones, let say $(q,M)$. Let $\sigma'$ be the sequence of transitions between these two configurations, it may read some letters ($w_p$) or not $w_p=\epsilon$, if it is exclusively composed of resets.
We pump $\sigma'$ which means that the pumped word is $w$ where $w_p$ has been removed.  

%Considérons un mot $w$ simplifié accepté par $\nu$-automate simplifié. Considérons une séquence de transition qui accepte $w$ de longueurs au moins $|Q|2^{|M|+|K|}+1$ dans ce cas on la séquence des configuration rencontré lors de la lecture de $w$ en contient deux identiques. On repèré la sequence de transitions entre ces deux configurations, on repère les caractères lus dans le mot dans ces transitions (éventuellement aucun si on pompe des resets), on pompe entre les deux. 

%------------------------------------------
\han{je suis ici}

We show that pumped word $w'.w''$, for $w=w'.w_p.w''$, with $w_p$ the sequence of letters read by pumped sequence $\sigma'$, is recognized by $A$, by induction on the number of loops.
%Montrons que le mot pompé est reconnu par le $\nu$-automate: si on rajoute des boucles (NOTE: pour notre théorème on veut supprimer la boucle mais autant faire un résultat plus général), on le fait par récurrence sur le nombre de boucles. Pour une boucle, c'est le mot de départ. Sinon, on montre que la séquence des configurations lors du parcours de la boucle est la même que lors du précédent passage de la boucle en considérant les transitions faites: 

- RESET: RAS

- READ $a$ dans v : on a pu franchir le read lors de l'itération précédente donc $a=t_v$ est bien en mémoire, on peut franchir à l'itération suivante

- WRITE $a$ dans v: si $a=k_v$ comme on a franchit la transition à l'étapte précédente on $t_v$ n'est pas dans la mémoire et donc on mémorise $t_v$ et on franchit la transition. Si $a$ est un token, ATTENTION il faut bien préciser que quand on pompe un mot, on met à jour les tokens sinon on lit deux fois le même token et on cela ne passe pas.

A l'issue de la boucle (que l'on en ait supprimé une ou rajouté), on suit les mêmes transition que celle du mot de départ pour arriver à un état acceptant. Il n'y a rien de particulier dans ce cas, tout se passe bien.

\end{proof}

Maintenant, on introduit un algorithme qui prend un mot accepté par un $\nu$-automate et le transforme en un mot de même longueur accepté par sa version simplifiée.


Algo:
Prendre une séquence de transition qui amène d'un état initial à un état acceptant pour la lecture de $w$ (NOTE: c'est cette séquence qui est importante, $w$ ne sera plus utilisé).

Poser $i=0$ et $w'=\epsilon$ et la configuration initiale $(q_0,M_0)$ où $q_0$ et $M_0$ sont l'état et la mémoire initiale de l'automate simplfiée.

On parcours les transitions:

si on lit un RESET on met à jour la configuration et on franchit la transition

si on lit un WRITE $v$: si $v$ est vide on pose $w'=w'k_v$ et on rajoute la clé en mémoire et on met l'état à jour en franchissant la transition. si $v$ contient sa clé, on fait $w'=w't_i$ et $i++$.

si on lit un READ $v$: on franchit la transition (on montrera dans la preuve après que l'on a le droit) en mettant à jour l'état et on pose $w'=w'k_v$.


\begin{lemma}\label{lem:correction-algo}
Si $w$ est reconnu par un $\nu$-automate alors $w'$ (qui le résultat de $w$ sur l'algo) est reconnu par la version simplifiée du $\nu$-automate.
\end{lemma}

\begin{proof}
On considère la séquence de transitions utilisée par l'algo et on montre qu'il a bien le droit de les franchir.

Pour le RESET pas de problème, on peut toujours franchir. Pour le WRITE $v$, si $v$ on peut stocker sa clé donc pas de problème, si $v$ contient sa clé, on utilise un token qui ne sera plus jamais utilisé car ne fait que croître. On rajoute une lettre à $w'$ qui est consommé dans la transition

Pour READ $v$: l'automate de départ peut franchir cette transition donc la mémoire de $v$ n'est pas vide. Donc à un moment, un caractère a été rajouté dans la variable $v$ (éventuellement, la lettre pouvant être dans la mémoire initiale) et il n'y a pas eu de RESET entretemps. Au moment où cette lettre a été ajouté dans $v$, dans l'automate simplifié on a ajouté $k_v$ (soit c'est dans la configuration initiale et dans ce cas $v$ contient $k_v$ par définition, soit on a fait un WRITE $v$ et dans ce cas soit $k_V$ est déjà dans la variable soit on l'y ajoute par le focntionnement de notre). L'automate simplifié peut donc traverser cette transition en consommant, le $k_v$ que l'on vien de rajouter à la fin de $w'$
\end{proof}

Voici un algo avec deux versions (une pour montrer que $\nu$NEP est dans PSPACE), une utile pour la preuve.

Initialisation:

Prend un $\nu$-automate simplifié

Soit un compteur $c$ sur $\log(|Q|)+|K|+1$ bits

Soit une configuration $(|\log(|Q|) +|K| bits)$ qui est la configuration initiale du $\nu$-automate.

optionnel: un mot $w=\epsilon$

Tant que l'état de la configuration n'est pas acceptant et que le compteur n'est pas à son maximum faire

Tirer au hasard une transition de l'automate

Si un RESET, on la franchit en mettant à jour l'état mémoire

Si un READ $v$, (OPTIONNEL on pose $w=wk_v$ et on consomme la lettre rajoutée) si on a $k_v$ est en mémoire dans $v$ on franchit et on met à jour la configuration sinon on s'arrête on rejette.

Si un WRITE $v$, on tire au hasard avec proba 1/2 (NOTE: la valeur de la proba n'est pas importante), (OPTIONNEL on pose $w=wt_{compteur}$ et on consomme le token rajoutée) on franchit la transition en mettant à jour l'état mais sans toucher à la mémoire, avec proba 1/2 (OPTIONNEL on pose $w=wk_v$ et on consomme la clé rajoutée) si $k_v$ est en mémoire, on s'arrête et on rejette sinon on traverse la transition ne mettant $k_v$ en mémoire.

\begin{lemma}\label{lem:empty-pspace}
 $\nu$NEP is in PSPACE.
\end{lemma}

\begin{proof}
Si l'automate n'est pas vide. Il contient un mot $w$, on le transforme en mot reconnu par l'automate simplifiée. On pompe ce pompe pour obtenir une séquence de transition et de configuration de taille bornée par $|Q|2^|K|$ qui amène d'un état initial à l'état finale. Notre algo a une proba strictement positivement de sélectionner cette séquence de transition, quand on fait un write l'algo a une proba strictement positivement de faire lire le même caractère. Si c'est choix aléatoire sont les bons alors La configuration mémorisée lors de notre algo suit la séquence de confiugraiton lors de la lecture de $w$. Comme la séquence de transition est bornée, on rencontrera l'état acceptant avant de s'arrêter. Il y a donc une chance strictement positive que notre algo accepte l'automate.

Supposons maintenant que si notre algo accepte alors on regarde le mot retournée par la partie optionnel de l'algo. Ce mot est accepté par le $\nu$-automate simplifié en suivant la séquence de transitions choisies aléatoirement devrait lors de l'algo. Un mot accepté par le $\nu$-automate simplifié est accepté par le $\nu$-automate de départ voir théorème précédent.

Notre algo termine toujours de plus la version sans la partie optionnelle est en espace polynomial donc  $\nu$NEP is in NPSPACE. Par le théorème de Savitch PSPACE=NPSPACE et donc on a $\nu$NEP is in PSPACE.

%By Savitch's theorem, we have PSPACE=NPSPACE. We consider an algorithm which memorizes: one restrained configuration and a counter on TODO bits. For each iteration, a transition starting from state TODO is selected randomly. If the transition is reset than the reset is done on the restrained memory. If the transition is a write than if the variable does not contain TODO then TODO is written otherwise TODO is written and the restrained memory is not unchanged. 
If the transition is a read and is TODO is in TODO then nothing is done otherwise the algorithm stop and reject. The counter is increased and if it reach TODO then the algorithm halts and reject. 
If TODO is not empty then there a words of length recognize by TODO. 
\end{proof}


==> HRA_example.tex <==
\node [draw, circle] (q0) {$q_0$};
\node [draw, circle, right = of q0] (q1) {$q_1$};
\node [draw, circle, double, right = of q1] (q2) {$q_2$};
\node [draw, circle, double, below = of q2] (q3) {$q_3$};

\draw [->, thick] (q0)--node[above]{$\emptyset/X$}(q1);
\draw [->, thick] (q1)--node[above]{$\emptyset/Y$}(q2);
\draw [->, thick] (q1)--node[below, rotate=-45]{$X/Y$}(q3);


==> hra-to-LaMA.tex <==

\node [draw, circle] (q0r) {$q_0$};
\node [draw, circle, right= of q0r] (q0w) {$q_0'$};
\node [draw, circle, right = of q0w] (q1r) {$q_1$};
\node [draw, circle, right = of q1r] (q1w) {$q_1'$};
\node [draw, circle, double, right = of q1w] (q2r) {$q_2$};
\node [draw, circle, below = of q1r] (q1w2) {$q_1''$};
\node [draw, circle, double, right = of q1w2] (q3r) {$q_3$};

\draw [->, thick] (q0r)--node[above]{$(\omega^1, \bold{w})$}node[below]{$(\omega^2,\bold{w})$}(q0w);
\draw [->, thick] (q0w)--node[above]{$(X^1,\bold{w})$}(q1r);
\draw [->, thick] (q1r)--node[above]{$(\omega^1, \bold{w})$}node[below]{$(\omega^2, \bold{w})$}(q1w);
\draw [->, thick] (q1w)--node[above]{$(Y^2, \bold{w})$}(q2r);
\draw [->, thick] (q1r)--node[above,rotate=-90]{$(X^1, \bold{r})$}node[below,rotate=-90]{$(\omega^2, \bold{w})$}(q1w2);
\draw [->, thick] (q1w2)--node[below]{$(Y^2, \bold{w})$}(q3r);

